A hybrid multi-time-step framework for pore-scale and continuum-scale modeling of solute transport in porous media

In this paper, we propose a computational framework,which is based on a domain decomposition technique, to employ both finite element method (which is a popular continuum modeling approach) and lattice Boltzmann method (which is a popular pore-scale modeling approach) in the same computational domain. To bridge the gap across the disparate length and time-scales, we first propose a new method to enforce continuum-scale boundary conditions (i.e., Dirichlet and Neumann boundary conditions) onto the numerical solution from the lattice Boltzmann method. This method are based on maximization of entropy and preserve the non-negativity of discrete distributions under the lattice Boltzmann method. The proposed computational framework allows different grid sizes, orders of interpolation, and time-steps in different subdomains. This allows for different desired resolutions in the numerical solution in different subdomains. Through numerical experiments, the effect of grid and time-step refinement, disparity of time-steps in different subdomains, domain partitioning, and the number of iteration steps on the accuracy and rate of convergence of the proposed methodology are studied. Finally, to showcase the performance of this framework in porous media applications, we use it to simulate the dissolution of calcium carbonate in a porous structure.

==> Sections/tmp/S2_old.tex <==
{\color {red}
If one
is inclined, more sophisticate models for boundaries can also
be employed, since they are in effect only with respect to solving
the Boltzmann equation. In the rest of this paper, we will use the 
following relations to model boundaries:
\begin{enumerate}[(i)]
\item \emph{Prescribed concentration boundary conditions (Dirichlet 
	boundary condition)}:~We will assume this portion
	of the boundary as a perfectly \emph{absorbing-emitting} boundary. 
	Let $\mathbf{x}\in\Gamma^{\mathrm{D}}$, and $\widehat{\mathbf{n}}(\mathbf{x})$ 
	be the outward normal at that point. We will define the following set:
	\begin{align}
	\label{Eqn:Gamma_D_neg}
		\Gamma^{\mathrm{D}}_{-} = \left\{ (\mathbf{x}, \boldsymbol{\zeta})
		\in \Gamma^{\mathrm{D}} \times \mathbb{R}^{n} \; \big| \; \widehat{\mathbf{n}}(\mathbf{x}) \cdot \boldsymbol{\zeta} < 0 \right\} 
	\end{align}
	Now we can write
	\begin{align}
	 	\mathrm{u}^{\mathrm{p}} (\mathbf{x}, \mathrm{t}) = 
		\int f(\mathbf{x},\boldsymbol{\zeta},\mathrm{t}) \; \mathrm{d} \zeta
		= \int_{\widehat{\mathbf{n}}(\mathbf{x})\cdot \boldsymbol{\zeta} < 0}
		f(\mathbf{x}, \boldsymbol{\zeta},\mathrm{t}) \; \mathrm{d}\boldsymbol{\zeta}
		+ \underbrace{\int_{\widehat{\mathbf{n}}(\mathbf{x})\cdot \boldsymbol{\zeta} \geq 0}f(\mathbf{x}, \boldsymbol{\zeta},\mathrm{t}) \; \mathrm{d}\boldsymbol{\zeta}}_{\tilde{\mathrm{u}}(\boldsymbol{x},\mathrm{t})}
	\end{align}
	where $\tilde{\mathrm{u}}(\mathbf{x},\mathrm{t})$ is the amount
	of matter absorbed by the boundary. We assume that $\Gamma^{\mathrm{D}}$ 
	be the interface between $\Omega$ and a reservoir at thermodynamic equilibrium. 		Hence, the distribution of the particles emitted from the boundary can
	be taken according to the Maxwell-Boltzmann distribution:
	\begin{align}
	\label{Eqn:Boltzmann_Dir}
		f(\mathbf{x},\boldsymbol{\zeta},\mathrm{t}) = \frac{1}{2} \max\{\mathrm{u}^{\mathrm{p}}(\mathbf{x}, \mathrm{t}) - \tilde{\mathrm{u}}(\mathbf{x},\mathrm{t}),0\}\frac{e^{-\boldsymbol{\zeta}\cdot\boldsymbol{\zeta}/2\mathrm{R}\mathrm{T}}}{\left( 2\pi \mathrm{R} \mathrm{T}\right)^{n/2}}  \quad \forall (\mathbf{x},\boldsymbol{\zeta}) \in \Gamma^{\mathrm{D}}_{-}
	\end{align}
	in which we have assumed the boundary to be stationary. The $\max$ operator
	is inserted due to the fact that the concentration cannot be negative. 
	Here, we have implicitly assumed that the particles do not interact, 
	and that they are classical particles. We will use this treatment for 
	enforcing the \emph{Dirichlet} boundary conditions.
	%
	\item \emph{Prescribed flux boundary conditions (Neumann boundary conditions)}:
	~In this case, we will 
	assume that the particles hitting the boundary are (immediately) reflected
	back into the domain $\Omega$. This assumption may not hold in reality,
	since a particle can accommodate on the boundary for an indefinite time
	and then be released into the domain at a later time. Furthermore, we will
	assume that the particles are classical and do not interact. Following
	a notation similar to the one given in Equation \eqref{Eqn:Gamma_D_neg}, 
	we may write:
	\begin{align}
	\label{Eqn:Boltmann_Neu}
		\big| \widehat{\mathbf{n}}\cdot \boldsymbol{\zeta}
		\big| f(\mathbf{x}, \boldsymbol{\zeta}, \mathrm{t}) = 
		\int_{\widehat{\mathbf{n}}\cdot \boldsymbol{\zeta}' > 0} 
		\mathcal{R}(\boldsymbol{\zeta},\boldsymbol{\zeta}') 
		\big| \widehat{\mathbf{n}}\cdot \boldsymbol{\zeta}'\big|
		f(\mathbf{x}, \boldsymbol{\zeta}', \mathrm{t}) \; \mathrm{d}\boldsymbol{\zeta}'
		+ {\color{red} \mathrm{q}^{\mathrm{p}} \frac{e^{-\boldsymbol{\zeta}\cdot\boldsymbol{\zeta}/2\mathrm{R}\mathrm{T}}}{(2 \pi \mathrm{R}\mathrm{T})^{n/2}}
		}
		\quad \forall (\mathbf{x},\boldsymbol{\zeta}) \in \Gamma^{\mathrm{N}}_{-}
	\end{align}
	where $\mathcal{R}(\boldsymbol{\zeta},\boldsymbol{\zeta}')$ is the 
	\emph{re-distribution kernel} \cite{1988_Cercignani_book}. Note that
	$(\mathbf{x},\boldsymbol{\zeta}')\in\Gamma^{\mathrm{N}}_{+}$. We have 
	assumed that the particles entering/leaving the domain are distributed
	according to the Maxwell-Boltzmann distribution. 
	%
	There are a multitude of choices available for the re-distribution kernel 
	depending on the particle-interface interaction model in use. 
	For instance, assuming elastic impact between the particles and 
	the boundary leads us to the following relation for the re-distribution
	kernel
	\begin{align}
	\label{Eqn:ReDist_Fac}
		\mathcal{R}(\boldsymbol{\zeta},\boldsymbol{\zeta}') = 
			\delta \left( \boldsymbol{\zeta}' - \boldsymbol{\zeta} + 
			2 (\widehat{\mathbf{n}}\cdot\boldsymbol{\zeta}) 
			\widehat{\mathbf{n}} \right)
	\end{align} 
	where $\delta(\cdot)$ is the Dirac delta. In this paper, we will
	solely use this choice for the re-distribution factor. Equation
	\eqref{Eqn:ReDist_Fac} leads to the \emph{bounce-back} condition,
	which is widely used in the lattice Boltzmann method. 
\end{enumerate}
To initialize the distribution of particles at time $\mathrm{t} = 0$,
we will use the equilibrium distribution given in Equation 
\eqref{Eqn:Maxwell_dist}. We can write:
\begin{align}
	f(\mathbf{x},\boldsymbol{\zeta};\mathrm{t}=0) = 
		f^{\mathrm{eq}.}(\mathbf{x},\boldsymbol{\zeta};\mathrm{t} = 0)
		\quad \forall (\mathbf{x},\boldsymbol{\zeta})\in\Omega \times 
		\mathbb{R}^{n}
\end{align}
This completes the statement of the Boltzmann equation. However, 
solving the Boltzmann equation is still a very difficult task and
cannot be accomplished without resorting to numerical methods.
In the next section, we will briefly review one of the most popular
methods for discretizing the Boltzmann equation.  
%-----------------------------;
% 	Lattice Boltzmann Method  ;
%-----------------------------;
\subsection{The lattice Boltzmann method}
A simple and yet popular way of discretizing the Boltzmann equation
is the lattice Boltzmann method. This method is essentially an
explicit finite difference discretization of Equation \eqref{Eqn:Boltzmann}.
Typically, the velocities (or equivalently, momentums) $\boldsymbol{\zeta}$
are discretized through a $DnQm$ lattice model, where $n$ is the number
of spatial dimensions and $m$ is the number of discrete velocities.
The population of particles that have velocity $\boldsymbol{e}_i$
at point $\mathbf{x}\in\Omega$ and time $\mathrm{t}$ will be denoted by 
$f_i(\mathbf{x},\mathrm{t})$ for every $i=1,\cdots,m$. We will consider
a spatial discretization by a uniform grid with spacing $\Delta x$. The
time-step will be denoted by $\Delta t$. The lattice Boltzmann equation
can be written as:
\begin{align}
\label{Eqn:LBE}
	\left.\big| f_i\right\rangle (\mathbf{x} + \boldsymbol{e}_i \Delta t,
	\mathrm{t} + \Delta t) = \left. \big| f_i \right \rangle (\mathbf{x},\mathrm{t})
	+ \boldsymbol{S} \left( \left.\big| f^{\mathrm{eq.}}_{i}\right\rangle(\mathbf{x},\mathrm{t}) - \left. \big| f_i\right \rangle (\mathbf{x}, \mathrm{t})\right)
\end{align}
where $\boldsymbol{S}$ is the $m\times m$ matrix
of relaxation-times and $\left.\big| \cdot \right\rangle$ is the $m \times 1$
array of the distributions at each lattice node and at each time-level.

In this paper, we are interested in using LBM to simulate advection-diffusion
processes. In the case of isotropic diffusion tensor (i.e., $\mathbf{D} = 
\mathrm{D}\mathbf{I}_{n}$ in Equation \eqref{Eqn:AD}), we shall take the relaxation
matrix as 
\begin{align}
	\boldsymbol{S} = \frac{1}{\tau} \mathbf{I}_{m}
\end{align}
where $\tau = 1/2 + \mathrm{D}/(c_s^2 \Delta t)$, with $c_s$ being the lattice
sound velocity. $\mathbf{I}_{m}$ is the identity matrix of size $m \times m$.
The equilibrium distribution will be
\begin{align}
\label{Eqn:Equi_Discrete}
	f^{\mathrm{eq}.}_{i}(\mathbf{x},\mathrm{t}) = \mathrm{u}(\mathbf{x},\mathrm{t})
	w_i \left( 1 + \frac{\boldsymbol{e}_i \cdot \mathbf{v}}{c_s^{2}}\right)
\end{align}
where $w_i$ is the weight associated with the velocity $\boldsymbol{e}_i$.
This class of LBMs are referred to as the Single-Relaxation-Time (SRT) 
methods. For more detail on this discretization, the reader should 
consult References \cite{1997_He_Luo_PRE, 2000_Lallemand_PRE,2001_Succi_LBM}. 
}

==> Sections/tmp/S3_Hybrid_LBM.tex <==
%************************************************;
%                                                ;
%  NAME                                          ;
%    S3_Hybrid_LBM.tex                           ;
%                                                ;
%  WRITTEN BY                                    ; 
%    Saeid Karimi                                ;
%    Kalyana Babu Nakshatrala                    ;
%                                                ;
%************************************************;
\section{PORE-SCALE MODELING: LATTICE BOLTZMANN METHODS}
\label{Sec:Hybrid_Pore-scale}
%
The Boltzmann equation provides a statistical description of 
the state of matter away from the thermodynamic equilibrium 
\citep{1988_Cercignani_book}. This equation describes the 
evolution of the distribution of particles in the phase 
space, from which macroscopic variables can be easily 
computed. If one neglects the external force term, the 
Boltzmann equation can be written as:
%--------------------------------;
%  Equation: Boltzmann equation  ;
%--------------------------------;
\begin{align}
  \label{Eqn:Boltzmann}
  \frac{\partial f}{\partial \mathrm{t}} 
  + \mathbf{v} \cdot \mathrm{grad}[f] 
  = \mathcal{Q}\left[ f,f^{\mathrm{eq}}\right]
\end{align}
%
where $f$ is the distribution function, $\mathbf{v}$ 
is the macroscopic (or background) velocity, and 
$\mathcal{Q}$ is the collision term. Herein, we 
will consider the Bhatnagar-Gross-Krook (BGK) 
collision model \citep{1954_BGK}, which can 
be written as:
%-----------------------;
%  Equation: BGK model  ;
%-----------------------;
\begin{align}
  \mathcal{Q}\left[ f,f^{\mathrm{eq}}\right] = \frac{1}{\lambda} (f^{\mathrm{eq}} - f)
\end{align}
%
where $f^{\mathrm{eq}}$ is the distribution of particles
in the phase space at the thermodynamics equilibrium. 
The parameter $\lambda$ is called the relaxation time. 
In this paper, we will use the Maxwell-Boltzmann distribution 
for the equilibrium distribution $f^{\mathrm{eq}}$. That is, 
%----------------------------------------------;
%  Equation: Equilibrium Maxwell distribution  ;
%----------------------------------------------;
\begin{align}
  \label{Eqn:MxBlt}
  f^{\mathrm{eq}}(\mathbf{x},\boldsymbol{\zeta};\mathrm{t})
  = \frac{\mathrm{u}(\mathbf{x},\mathrm{t})}{\sqrt{2 \pi \mathrm{R}
      \mathrm{T}}} \mathrm{exp}\left( -\frac{(\boldsymbol{\zeta} - 
    \mathbf{v})\cdot (\boldsymbol{\zeta} - \mathbf{v})}{2\mathrm{R}\mathrm{T}}
  \right)
\end{align}
%
where $\mathrm{u}(\mathbf{x},t)$ is the concentration, 
$\mathrm{R}$ is the ideal gas constant, and $\mathrm{T}$ 
is the temperature. The velocity of particles is shown 
by $\boldsymbol{\zeta}$.  

{\color{red}
In order to provide a complete description of the Boltzmann
equation for a physical problem, appropriate boundary conditions
have to be included. Fortunately, the mathematical theory of 
boundary conditions for Boltzmann equation is rather well-developed
; e.g. see References \citep{1971_Cercignani_Lampis, 1988_Cercignani_book,
2013_Cercignani_book}. However, to use the existing theories to their
full extent, one has to incorporate detailed dynamics for interaction
between the particle and the surrounding surface of the domain.
Obviously, the continuum model problem given in Equation \eqref{Eqn:AD}
lacks such information. Hence, the Boltzmann equation provides a 
much more powerful framework to account for detailed dynamics of
gas-surface interaction that the continuum model is incapable of.
In this paper, we will assume that the user merely intends to replicate
the behavior of the macroscopic solution of Equation \eqref{Eqn:AD}
and in-depth treatment of gas-surface interaction is of no interest.

A popular numerical method for solving the Boltzmann equation for
complex hydrodynamics simulations is the lattice Boltzmann method
\citep{1997_He_Luo_PRE,2000_Lallemand_PRE, 2001_Succi_LBM}. LBM has
an explicit structure and is natural to parallelize. However, it
fails to preserve some important mathematical properties of the 
advection-diffusion equation \citep{2015_Karimi_LBM}. In order 
to avoid spurious results, we will employ Entropic Lattice 
Boltzmann Method (ELBM) \citep{2002_Karlin,2006_Karlin}. Using 
ELBM, one can make sure that the path of the system toward
thermodynamic equilibrium is such that the entropy increases 
monotonically. As a result, the resulting distribution of particles
from numerical solution will be non-negative. To achieve this
goal, we need to choose an appropriate entropy function. In the following 
section, we will provide a ELBM discretization of Equation 
\eqref{Eqn:Boltzmann} base on References \citep{2002_Karlin,2006_Karlin}, 
along with a new method to enforce boundary conditions in \eqref{Eqn:AD} 
inspired by Reference \citep{2015_Dottori}.

%=====================================================;
%  Subsection: The entropic lattice Boltzmann method  ;
%=====================================================;
\subsection{The entropic lattice Boltzmann method}
\label{Sec:Hybrid_Pore_Scale_ELBM}
In this section, we will provide an overview of ELBM with 
BGK collision model. The main purpose of ELBM is to guarantee
monotonicity in entropy production. The lattice model for 
discretization of a $n$-dimensional space and $m$ discrete
velocity components will be denoted by $DnQm$ (see Figure
\ref{Fig:lattice} for the case of $D2Q9$ lattice). The lattice
cell-size will be shown by $\Delta x$ and time-step by $\Delta t$.
We will use the Dirac notation $\left \langle \cdot \big| \right.$ and 
$\left. \big| \cdot \right \rangle$ to show row and column vectors 
respectively.
%
Discretization of Equation \eqref{Eqn:Boltzmann} under ELBM will 
be as follows
\begin{align}
	\label{Eqn:ELBM}
	f_{i}(\mathbf{x} + \boldsymbol{e}_i \Delta t, \; t + \Delta t)
	= f_{i} (\mathbf{x},t) + \frac{\alpha \beta}{\tau} \left( f_{i}^{\mathrm{eq.}}
	(\mathbf{x},t) - f_i (\mathbf{x},t)\right)
\end{align}
where $f_i$ is the population with velocity $\boldsymbol{e}_i,\;i=1,\cdots,m$.
The non-dimensional relaxation time is shown by $\tau$ and is taken to be
$\tau = 1/2 + \mathrm{D}/c_s^2 \Delta t$, where $c_s$ is the lattice 
sound velocity. The discrete equilibrium distribution is $f_i^{\mathrm{eq.}}$
and is an approximation of the Maxwell-Boltzmann distribution given in 
Equation \eqref{Eqn:MxBlt}. That is
\begin{align}
	f_{i}^{\mathrm{eq.}} (\mathbf{x},t) = \mathrm{u}(\mathbf{x},t) \varphi_i
\end{align}
where the coefficient $\varphi_i$ is defined as
\begin{align}
	\varphi_i = w_i \left( 1 + \frac{\boldsymbol{e}_i \cdot \mathbf{v}}{c_s^{2}} + 
	\frac{1}{2} \frac{(\boldsymbol{e}_i \cdot \mathbf{v})^2}{c_s^{4}}
	- \frac{\mathbf{v}\cdot \mathbf{v}}{c_s^2}\right)
\end{align}
where $w_i$ is the weight associated with discrete velocity $\boldsymbol{e}_i$.
In this paper, we will assume that $\left\| \mathbf{v} \right\| \ll c_s$ in the 
entire computational domain.
%
Here on, we shall denote the discrete collision term as $\mathcal{Q}_i(\mathbf{x}, t)
= \left( f_{i}^{\mathrm{eq.}}(\mathbf{x},t) - f_i (\mathbf{x},t)\right)/\tau$.
%
In Equation \eqref{Eqn:ELBM}, $\alpha$ is the root of the following non-linear
equation if the system is away form thermodynamic equilibrium
\begin{align}
\label{Eqn:alpha}
	\mathcal{H}\left( \left. \big| f_i \right\rangle \right) \big|_{(\mathbf{x},t)}
	= \mathcal{H} \left( \left. \big| f_i \right \rangle 
	+ \alpha \left. \big| \mathcal{Q}_i \right \rangle \right) \big|_{(\mathbf{x},t)}
\end{align}
otherwise, $\alpha = 2$. In Equation \eqref{Eqn:alpha}, $\mathcal{H}$ 
is the Boltzmann function and is defined as follows
\begin{align}
\label{Eqn:H}
	\mathcal{H}(\left.\big| f_i \right \rangle)\big|_{(\mathbf{x},t)}
	= \sum_{i = 1}^{m} f_i(\mathbf{x},t) \log\left( 
	\frac{f_i(\mathbf{x},t)}{\varphi_i}\right)
\end{align}
Parameter $\beta$ in Equation \eqref{Eqn:ELBM} belongs to the interval
$(0,1)$. The physical interpretation of this procedure is illustrated in
Figure \ref{Fig:ELBM}. In the following we will provide a new method
for enforcing Dirichlet- and Neumann-type boundary conditions in Equation
\eqref{Eqn:AD}. For brevity, we will use the following notation
\begin{align}
\label{Eqn:Boundary_Vel}
	\mathsf{M}^{-} (\mathbf{x}) := \left\{ 
	i \big| \; \boldsymbol{e}_i \cdot \widehat{\mathbf{n}}(\mathbf{x})
	< 0,\; i=1,\cdots,m \; \text{and} \; \mathbf{x}\in \partial \Omega \right\}
\end{align}
where $\widehat{\mathbf{n}}(\mathbf{x})$ is the unit outward normal to $\partial \Omega$.
Obviously, the unknown populations near the boundary are $f_i$ with $\boldsymbol{e}_i
\in \mathsf{M}^{-}(\mathbf{x})$ for every point $\mathbf{x}$ on $\partial \Omega$. 
The rest of the discrete populations are known from the collision and streaming steps 
prior to enforcement of boundary conditions. However, note that the Dirichlet and 
Neumann boundary conditions given in Equation \eqref{Eqn:AD}, are the valid 
boundary conditions for the advection-diffusion equations and not the 
Boltzmann equation \citep{2002_Karlin_BC}.
\begin{enumerate}[(a)]
\item \emph{Dirichlet boundary condition}:~Let $\mathbf{x} \in \Gamma^{\mathrm{D}}$
and $\mathrm{u}^{\mathrm{p}}(\mathbf{x},t)$ be the prescribed concentration at that
point. The unknown populations will be found using the following relation
\begin{align}
\label{Egn:LBM_Dir}
	&\min_{f_j,\;j\in \mathsf{M}^{-}(\mathbf{x})} \; \mathcal{H}\left( \left. \big| 
	f_i \right \rangle \right) \big|_{(\mathbf{x},t)} \nonumber \\
	&\text{subject to} \; \sum_{i = 1}^{m} f_i (\mathbf{x},t) = \mathrm{u}^{\mathrm{p}}(\mathbf{x},t)
\end{align}
where the function $\mathcal{H}$ is defined in Equation \eqref{Eqn:H}. This minimization
problem will result in the following relation
\begin{align}
	&f_i (\mathbf{x},t) = \frac{\varphi_{i}}{\sum_{j\in \mathsf{M}^{-}(\mathbf{x})} \varphi_j}
		\left( \mathrm{u}^{\mathrm{p}}(\mathbf{x},t) - \sum_{k \nin \mathsf{M}^{-}(\mathbf{x})}
		f_k (\mathbf{x},t)\right) \quad i \in \mathsf{M}^{-}(\mathbf{x}) \nonumber \\
		&f_i(\mathbf{x},t) \geq 0 \quad \forall i = 1,\cdots,m
\end{align}
Note that the function $\mathcal{H}$ is only defined for non-negative arguments.
\item \emph{Neumann boundary condition}:~Let $\mathbf{x}\in \Gamma^{\mathrm{N}}$ and 
$\mathrm{q}^{\mathrm{p}}(\mathbf{x},t)$ be the prescribed flux at that point. The 
unknown populations will be found as
\begin{align}
\label{Eqn:LBM_Neu}
	&\min_{f_j,\;j\in \mathsf{M}^{-}(\mathbf{x})} \; 
	\mathcal{H}(\left. \big| f_i \right \rangle)\big|_{(\mathbf{x},t)} \nonumber \\
	&\text{subject to} \; \sum_{i = 1}^{m} f_i(\mathbf{x},t) \boldsymbol{e}_i \cdot 
	\widehat{\mathbf{n}}(\mathbf{x}) = \mathrm{q}^{\mathrm{p}}(\mathbf{x},t)
\end{align}
with $\widehat{\mathbf{n}}(\mathbf{x})$ being the unit outward normal defined earlier.
This minimization problem will result in a non-linear equation in terms of Lagrange multiplier
for the hydrodynamic constraint:
\begin{align}
	\sum_{i \in \mathsf{M}^{-}(\mathbf{x})} \varphi_i (\boldsymbol{e}_i \cdot \widehat{
	\mathbf{n}}(\mathbf{x})) \mathrm{exp}\left( -1 - \gamma \left( \boldsymbol{e}_i 
	\cdot \widehat{\mathbf{n}}(\mathbf{x})\right)\right) = \mathrm{q}^{\mathrm{p}}
	(\mathbf{x},t) - \sum_{j \nin \mathsf{M}^{-}(\mathbf{x})} (\boldsymbol{e}_j \cdot 
	\widehat{\mathbf{n}}(\mathbf{x})) f_j (\mathbf{x},t)
\end{align}
where $\gamma$ is the Lagrange multiplier. Once the value of $\gamma$ is known, the 
populations can be found using the following relation:
\begin{align}
	f_i(\mathbf{x},t) = \varphi_i \mathrm{exp}\left( -1 - \gamma \left( \boldsymbol{e}_i 
	\cdot \widehat{\mathbf{n}}(\mathbf{x})\right)\right) \quad i\in\mathsf{M}^{-}(\mathbf{x})
\end{align}
which guarantees non-negative values for $f_i$. In the case of one-dimensional
lattice models (e.g. the $D1Q2$ lattice), this method reduces to the conventional
bounce-back method.
\end{enumerate}
Through this method of enforcing boundary conditions, which is based on maximization of
entropy, we ensure monotonic increase in entropy. The physical interpretation of this
method is that the system in $\Omega$ is connected to systems in thermodynamic equilibrium.
The adjacent systems connected to $\Omega$ through $\Gamma^{\mathrm{D}}$ and 
$\Gamma^{\mathrm{N}}$ are in different states of thermodynamic equilibrium. Minimization
of the function $\mathcal{H}$ ensures that the equilibrium condition for particles near the 
boundary is respected. The constraints in Equations \eqref{Egn:LBM_Dir} and \eqref{Eqn:LBM_Neu}
are the macroscopic hydrodynamic conditions of the system at the respective points of the 
domain.
}


==> Sections/tmp/S4_Proposed_coupling_old.tex <==
%-----------------------------------------------;
% 	Section 3: Proposed coupling
% 	By: Saeid Karimi, Kalyana Babu Nakshatrala
%-----------------------------------------------;
\section{PROPOSED COUPLING ALGORITHM}
\label{Sec:Coupling}
In this section the proposed coupling method for
hybrid FEM-LBM computation will be presented. 
The current method allows different time-steps
and grid size for FEM and LBM domains. This method
is an iterative scheme and uses overlapping domain
partitioning. We will follow the notation employed in
Equation \eqref{Eqn:AD}.

Consider a bounded and open domains $\Omega_{\mathrm{FEM}}$
and $\Omega_{\mathrm{LBM}}$ such that $\Omega_{\mathrm{FEM}}
\cup \Omega_{\mathrm{LBM}} = \Omega$ and $\Omega_{\mathrm{FEM}}
\cap \Omega_{\mathrm{LBM}} \neq \emptyset$. 
We will use the finite element discretization in domain
$\Omega_{\mathrm{FEM}}$ and a uniformly spaced lattice 
in $\Omega_{\mathrm{LBM}}$. The region 
$\Omega_{\mathrm{FEM}}\cap \Omega_{\mathrm{LBM}}$ is called
the buffer zone. Figure \ref{Fig:Overlap} shows a pictorial 
description of the such partitioning. We shall denote the 
boundaries of the buffer zone by $\tilde{\Gamma}_{\mathrm{FEM}}$
and $\tilde{\Gamma}_{\mathrm{LBM}}$ (as shown in Figure \ref{Fig:Overlap}). 
Furthermore, we will take
\begin{align}
 	\partial \Omega_{\mathrm{FEM}} = \Gamma_{\mathrm{FEM}} 
	\cup \tilde{\Gamma}_{\mathrm{FEM}}, \quad
	\partial \Omega_{\mathrm{LBM}} = \Gamma_{\mathrm{LBM}} 
	\cup \tilde{\Gamma}_{\mathrm{LBM}}
\end{align}
We will enforce Nuemann 
type boundary conditions on $\tilde{\Gamma}_{\mathrm{FEM}}$ 
and $\tilde{\Gamma}_{\mathrm{LBM}}$. Concentration in the 
FEM domain will be denoted by $\mathrm{u}_{\mathrm{FEM}}$
and concentration in the LBM domain will be shown by 
$\mathrm{u}_{\mathrm{LBM}}$. Hence, the governing partial 
differential equations in each domain can be written as
\begin{subequations}
\label{Eqn:Coupling_PDE}
	\begin{align}
		\text{FEM domain:}\; \left\{ 
			\begin{array}{l c}
				\partial \mathrm{u}_{\mathrm{FEM}}/\partial \mathrm{t} + 
				\mathrm{div}\left[ \mathbf{v} \mathrm{u}_{\mathrm{FEM}} - 
				\mathbf{D} \mathrm{grad}\left[ \mathrm{u}_{\mathrm{FEM}}\right]\right]
				= \mathrm{s} \quad &(\mathbf{x}, \mathrm{t})\in 
				\Omega_{\mathrm{FEM}}\times\mathcal{I} \\
				\mathrm{u}_{\mathrm{FEM}} = \mathrm{u}_{0} \quad &\mathbf{x}\in \Omega_{\mathrm{FEM}},\;
				\mathrm{t} = 0  \\
				\mathrm{u}_{\mathrm{FEM}} = \mathrm{u}^{\mathrm{p}} \quad &\mathbf{x} \in \Gamma_{\mathrm{FEM}} \cap \Gamma^{\mathrm{D}},\; \mathrm{t} \in \mathcal{I} \\
				\widehat{\mathbf{n}}\cdot\left( \mathbf{v}\mathrm{u}_{\mathrm{FEM}}
				- \mathbf{D} \mathrm{grad}[\mathrm{u}_{\mathrm{FEM}}]\right) = 
				\mathrm{q}^{\mathrm{p}} \quad &\mathbf{x}\in \Gamma_{\mathrm{FEM}}\cap
				\Gamma^{\mathrm{N}},\;\mathrm{t} \in \mathcal{I} \\
				\widehat{\mathbf{n}}\cdot\left( \mathbf{v}\mathrm{u}_{\mathrm{FEM}}
				- \mathbf{D} \mathrm{grad}[\mathrm{u}_{\mathrm{FEM}}]\right) = 
				\chi_{\mathrm{LBM}\rightarrow\mathrm{FEM}} \quad &\mathbf{x}\in \tilde{\Gamma}_{\mathrm{FEM}},\;\mathrm{t} \in \mathcal{I}
			\end{array}
		\right. \\
	\text{LBM domain:}\; \left\{ 
	\begin{array}{l c}
				\partial \mathrm{u}_{\mathrm{LBM}}/\partial \mathrm{t} + 
				\mathrm{div}\left[ \mathbf{v} \mathrm{u}_{\mathrm{LBM}} - 
				\mathbf{D} \mathrm{grad}\left[ \mathrm{u}_{\mathrm{LBM}}\right]\right]
				= \mathrm{s} \quad &(\mathbf{x}, \mathrm{t})\in 
				\Omega_{\mathrm{LBM}}\times\mathcal{I} \\
				\mathrm{u}_{\mathrm{LBM}} = \mathrm{u}_{0} \quad &\mathbf{x}\in \Omega_{\mathrm{LBM}},\;
				\mathrm{t} = 0  \\
				\mathrm{u}_{\mathrm{LBM}} = \mathrm{u}^{\mathrm{p}} \quad &\mathbf{x} \in \Gamma_{\mathrm{LBM}} \cap \Gamma^{\mathrm{D}},\; \mathrm{t} \in \mathcal{I} \\
				\widehat{\mathbf{n}}\cdot\left( \mathbf{v}\mathrm{u}_{\mathrm{LBM}}
				- \mathbf{D} \mathrm{grad}[\mathrm{u}_{\mathrm{LBM}}]\right) = 
				\mathrm{q}^{\mathrm{p}} \quad &\mathbf{x}\in \Gamma_{\mathrm{LBM}}\cap
				\Gamma^{\mathrm{N}},\;\mathrm{t} \in \mathcal{I} \\
				\widehat{\mathbf{n}}\cdot\left( \mathbf{v}\mathrm{u}_{\mathrm{LBM}}
				- \mathbf{D} \mathrm{grad}[\mathrm{u}_{\mathrm{LBM}}]\right) = 
				\chi_{\mathrm{FEM}\rightarrow\mathrm{LBM}} \quad &\mathbf{x}\in \tilde{\Gamma}_{\mathrm{LBM}},\;\mathrm{t} \in \mathcal{I}
			\end{array}
	\right. \\
	{\color {red}
	\text{LBM domain:}\; \left\{ 
		\begin{array}{l c}
			\partial f/\partial \mathrm{t} + \mathbf{v} \cdot \mathrm{grad}[f]
			= \left( f^{\mathrm{eq.}} - f\right)/\lambda \quad &\mathbf{x}\in\Omega_{\mathrm{LBM}},\;\mathrm{t}\in\mathcal{I} \\
			f = f_0 \quad &\mathbf{x}\in\Omega_{\mathrm{LBM}},\;\mathrm{t}=0 \\
			\mathrm{u} = \mathrm{u}^{\mathrm{p}}
			\quad &\mathbf{x} \in \Gamma_{\mathrm{LBM}} \cap \Gamma^{\mathrm{D}},\; \mathrm{t} \in \mathcal{I} \\
			\mathbf{q}\cdot
			\widehat{\mathbf{n}} = \mathrm{q}^{\mathrm{p}} \quad &\mathbf{x}\in \Gamma_{\mathrm{LBM}}\cap \Gamma^{\mathrm{N}},\;\mathrm{t} \in \mathcal{I} \\
			\mathbf{q}\cdot
			\widehat{\mathbf{n}} = \chi_{\mathrm{FEM}\rightarrow\mathrm{LBM}} \quad &\mathbf{x}\in \tilde{\Gamma}_{\mathrm{LBM}},\;\mathrm{t} \in \mathcal{I}
		\end{array}
	\right.
	}
	\end{align}
\end{subequations}
where $\chi_{\mathrm{LBM}\rightarrow\mathrm{FEM}}$ is the flux 
calculated from the LBM domain and applied to the FEM domain.
$\chi_{\mathrm{FEM}\rightarrow\mathrm{LBM}}$ is the flux imposed
on the LBM domain from the FEM domain.
{\color {red} The distribution of particles is denoted by $f$, which 
is a function of position $\mathbf{x}$, momentum $\mathbf{p}$ and 
time $\mathrm{t}$.  The initial distribution of particles is 
denoted by $f_0$ and the relaxation time is $\lambda$. 
The equilibrium distribution is shown by $f^{\mathrm{eq.}}$.
The source term in the Boltzmann equation is ignored. We have used the 
following definitions:
\begin{subequations}
\begin{align}
	\mathrm{u} = \lim_{\delta \rightarrow 0} \frac{\int_{-\infty}^{\infty} \int_{\mathcal{B}_{\mathbf{x}}\cap \Omega_{\mathrm{LBM}}} f \; \mathrm{d}\Omega \; \mathrm{d}^{n} \mathbf{p}}{\int_{\mathcal{B}_{\mathbf{x}}\cap \Omega_{\mathrm{LBM}}}\mathrm{d}\Omega} \quad \text{and} \quad
	\mathbf{q} = \lim_{\delta \rightarrow 0} \frac{\int_{-\infty}^{\infty} \int_{\mathcal{B}_{\mathbf{x}}\cap \Omega_{\mathrm{LBM}}} f\mathbf{p}/m \; \mathrm{d} \Omega \; \mathrm{d}^{n} \mathbf{p}}{\int_{\mathcal{B}_{\mathbf{x}}\cap \Omega_{\mathrm{LBM}}}\mathrm{d}\Omega}
\end{align}
\end{subequations}
where $\mathcal{B}_{\mathbf{x}}$ is an open ball centered at 
$\mathbf{x}$ and with a radius of $\delta$.The mass of particles is
shown by $m$.
}{\color {blue} \emph{ I'm not quite sure about these definitions. It needs
more thinking}.}

By imposing Neumann conditions on $\tilde{\Gamma}_{\mathrm{LBM}}$ and 
$\tilde{\Gamma}_{\mathrm{FEM}}$, we can hope to achieve better mass 
balance properties than Neumann-Dirichlet or Dirichlet-Dirichlet 
alternatives. The concentration $\mathrm{u}$ in the buffer zone
can be computed as 
\begin{align}
	\mathrm{u} = \beta(\mathbf{x}) \mathrm{u}_{\mathrm{FEM}} + (1-\beta(\mathbf{x}))
	\mathrm{u}_{\mathrm{LBM}} \quad \mathbf{x} \in \Omega_{\mathrm{FEM}}\cap
	\Omega_{\mathrm{LBM}}
\end{align}
where $\beta(\mathbf{x})$ is an interpolation function satisfying
$\beta(\mathbf{x}\in\tilde{\Gamma}_{\mathrm{LBM}}) = 0$ and 
$\beta(\mathbf{x}\in\tilde{\Gamma}_{\mathrm{FEM}}) = 1$.

In this paper, we will use FEM to compute for the coarse features 
of the solution and in regions where more a more detailed solution 
is required LBM is employed. Hence, we assume that the time-step
used for integration of the FEM domain, $\Delta t_{\mathrm{FEM}}$, 
is larger than that of LBM, $\Delta t_{\mathrm{LBM}}$. 











